VLG-CBM: Training Concept Bottleneck Models with Vision-Language Guidance

Concept Bottleneck Models (CBMs) provide interpretable prediction by introducing an intermediate Concept Bottleneck Layer (CBL), which encodes human-understandable concepts to explain models' decision. Recent works proposed to utilize Large Language Models and pre-trained Vision-Language Models to automate the training of CBMs, making it more scalable and automated. However, existing approaches still fall short in two aspects: First, the concepts predicted by CBL often mismatch the input image, raising doubts about the faithfulness of interpretation. Second, it has been shown that concept values encode unintended information: even a set of random concepts could achieve comparable test accuracy to state-of-the-art CBMs. To address these critical limitations, in this work, we propose a novel framework called Vision-Language-Guided Concept Bottleneck Model (VLG-CBM) to enable faithful interpretability with the benefits of boosted performance. Our method leverages off-the-shelf open-domain grounded object detectors to provide visually grounded concept annotation, which largely enhances the faithfulness of concept prediction while further improving the model performance. In addition, we propose a new metric called Number of Effective Concepts (NEC) to control the information leakage and provide better interpretability. Extensive evaluations across five standard benchmarks show that our method, VLG-CBM, outperforms existing methods by at least 4.27% and up to 51.09% on Accuracy at NEC=5 (denoted as ANEC-5), and by at least 0.45% and up to 29.78% on average accuracy (denoted as ANEC-avg), while preserving both faithfulness and interpretability of the learned concepts as demonstrated in extensive experiments.

==> src/futurework.tex <==
\label{sec:limit}

Despite the superior performance of our proposed \algoname~over prior work, as demonstrated by extensive experiments, one potential limitation is the reliance on large pretrained models (e.g. the success of open-domain grounded object detection model that we use to enforce vision guidance). Nevertheless, prior work (e.g. Labo, LM4CV, LF-CBM) shared similar limitation on the reliance of large pre-trained models (e.g. CLIP). Nevertheless, on the other hand, it also means that our techniques have the potential to be further improved with the advancement of large pre-trained models, which are the trend and becoming essential for deep learning. We will leave it as future work 

% we think this is a very exciting direction and the limitation will be alleviated 
% as the foundation models 


% are also limited by the laar

% One potential limitation of our proposed technique in Sec 3 is that our current success 

% In this work, we have made the first attempt to utilize the open-domain grounded object detection model to help on the vision supervision. Our current success is building upon the success of the 

% However, currently it may not directly work for the domains that has very different distributions than 

% (e.g. medical images), and it would require to develop 
% To extend our work to other vision domains (e.g. medical images), it would require to develop  

==> src/problem_formulation.tex <==
The Concept Bottleneck Model (CBM) introduces an intermediate concept bottleneck layer (CBL), where each neuron represents a human-understandable concept. CBL is followed by an interpretable final prediction layer, which predicts the label of input relying on the concept prediction from CBL. Formally, let $z = l(x)$ be the feature representation generated by the backbone. Denote the CBL concept prediction as $c(z)$ and the final prediction layer as $h(\cdot)$. The final class prediction of the CBM is thus $\hat{y} = h(c(z)) = h \circ c \circ l(x)$. 

Under this setting, the key problem in training a CBM is training the concept bottleneck layer $c$: how to train a CBL so that each neuron $c_i$ corresponds to an interpretable concept $a_i$. Original CBM uses human-specified labels and trains the CBL in a supervised way. Recently, Lable-Free CBM and LaBo proposed to utilize Large Language Models (LLM) to generate a set of concepts $\{a_i\}$, then train CBL to be aligned with these concepts with the guidance of vision language models (e.g. CLIP). 

Previous works suggest that different models may use different features to make predictions. While for current CBMs, the collected concepts are agnostic to models. We argue that model-specific information should be exploited when choosing the concept set. 

\begin{itemize}
    \item We plan to use large segmentation models to obtain concepts from images  
\end{itemize}
